Integration of Formal Proof into Unified Assurance Cases with Isabelle/SACM

Assurance cases are often required to certify critical systems. The use of formal methods in assurance can improve automation, increase confidence, and overcome errant reasoning. However, assurance cases can never be fully formalised, as the use of formal methods is contingent on models that are validated by informal processes. Consequently, assurance techniques should support both formal and informal artifacts, with explicated inferential links between them. In this paper, we contribute a formal machine-checked interactive language, called Isabelle/SACM, supporting the computer-assisted construction of assurance cases compliant with the OMG Structured Assurance Case Meta-Model. The use of Isabelle/SACM guarantees well-formedness, consistency, and traceability of assurance cases, and allows a tight integration of formal and informal evidence of various provenance. In particular, Isabelle brings a diverse range of automated verification techniques that can provide evidence. To validate our approach, we present a substantial case study based on the Tokeneer secure entry system benchmark. We embed its functional specification into Isabelle, verify its security requirements, and form a modular security case in Isabelle/SACM that combines the heterogeneous artifacts. We thus show that Isabelle is a suitable platform for critical systems assurance.

==> sec/isacm-old.tex <==
In this section we introduce a textual concrete syntax for the \ac{sacm} ontology as well as a tool support 
for machine verified assurance cases called \isacm. This allows us to use \ac{sacm} as a 
domain-specific modeling language in Isabelle.

Our approach gives a concrete syntax for \ac{sacm} in terms of Isabelle commands as follows:
\begin{enumerate*} 
   \item instances of abstract classes in the metamodel do not have concrete syntax.
   \item instances of concrete leaf child classes in the metamodel have concrete syntax 
         consisting of an Isabelle blue command. 
         The cammand has the name of the represented leaf child class. 
   \item instances of attributes of a leaf child class, including the inherited once from parent 
         classes, have a 
         concrete syntax represented by an Isabelle green command. The command has the name of 
         the represented attribute.
   \item instances of asscociations between leaf child classes has a concrete syntax represented 
         by an Isabelle green command. The command has the name of the represented association and
         has an input with the type of the associate of the underlying instance.
   \item instances of associations between the concrete classes and abstract classes have no concrete syntax.
         However, we generate those associations automatically behind the sceans. 
         The generation is done following the semantics of the \ac{sacm} ontology.
\end{enumerate*}

For the case of the class \inlineisar+Claim+ from the \inlineisar+ArgumentationPackage+
the concrete syntax is: 
\begin{isar}[numbers=none, backgroundcolor=\color{black!10}, frame=lines]
(*@\textcolor{Blue}{CLAIM}@*) <claim_gid> 
(*@\textcolor{OliveGreen}{isABS}@*) (*@\textcolor{OliveGreen}{isCIT}@*)
(*@\textcolor{OliveGreen}{CONTENT}@*) <MultiLangString>
\end{isar}
\begin{wrapfigure}{r}{0.40\linewidth}
  \vspace{-5.5ex}

  \centering
  \includegraphics[width=4.8cm]{Figures/ClaimA_DSL}

  \vspace{-2.5ex}
  
  \caption{Concrete syntax for a claim in \isacm}
  
  \label{fig:Claim_A}

  \vspace{-6ex}
\end{wrapfigure}
\dots where the place holders are explained in more details in the sequel. Note that 
\textcolor{OliveGreen}{\inlineisar+isABS+} and \textcolor{OliveGreen}{\inlineisar+isCIT+}  are
optional keywords and they are modeling the attributes \inlineisar+isAbstract+ and \inlineisar+isCitation+
inherited from the \inlineisar+BasePackage+ of \ac{sacm} metamodel. \textcolor{OliveGreen}{\inlineisar+CONTENT+} 
models an instance of the association \inlineisar+content_assoc:: MultiLangString+ which assciate
the class \inlineisar+Claim+ to the class \inlineisar+MultiLangString+. 

\autoref{fig:Claim_A}, shows a screenshot from \isacm. It is a plugin extending \idof with the 
concrete syntax for \ac{sacm}. Behind the sceans, the syntax is immidiatly compiled away
and evaluated by \ipide which adds, in the case of successful evaluation,
a list of automatically generated \textcolor{Blue}{\inlineisar+text*+}. For example, one of
the \textcolor{Blue}{\inlineisar+text*+} that is automatically generated after writing
the syntax of claim on a top of \isacm is 
\textcolor{Blue}{\inlineisar+text*+}\inlineisar+[Claim_A+\inlineisar+:: Claim, +\inlineisar+isCitation= True,+\inlineisar+ isAbstract= True+
\inlineisar+, assertionDeclaration+\inlineisar+ = NeedSupport]+
\inlineisar+\<open>Description in multiple language\<close>+.
The latter instance can be
referenced inside text areas, \ie{} \inlineisar+text+ or \textcolor{Blue}{\inlineisar+text*+},  
using the antiquotations as follows \inlineisar+text\<open>+ \inlineisar+@{Claim Claim_A}\<close>+. 
The reference is in the form of a hyperlink that one can click on and jump to the exact line 
where the claim was defined. Additionally one can hover on the
reference to get a pop-up with more details on the reference (\eg, the type of the reference). 
These machine verified references is very useful for the 
consistancy, the maintanance and the review of the assurance case and any kind of document.
Which may save a lot of effort in certification processes.
\begin{wrapfigure}{r}{0.70\linewidth}
  \vspace{-5.5ex}

  \centering
  \includegraphics[width=5.2cm]{Figures/Rel_DSL}

  \vspace{-2.5ex}
  
  \caption{Concrete syntax for a claim in \isacm}
  
  \label{fig:ClaimA_DSL}

  \vspace{-6ex}
\end{wrapfigure}

For the case where the evaluation of the syntax  does not succeed,
the user will get an error from \ipide as shown in~\autoref{fig:ClaimA_DSL}. 
The top error is related to the red line under the command \textcolor{Blue}{\inlineisar+ASEERTED_INFERENCE+}.
One can hover on the command to pop-up a panel with the details of the error. 
The top error state that no claim with name \inlineisar+Claim_B+ 
exist within the underlying theory context. An alternative
to check the error is the usage of the output panel in Isabelle's user interface. 
If one tries to reference the non succefully compiled
command by an antiquotation as in \inlineisar+text\<open>+ \inlineisar+@{AssertedInference Rel_A}\<close>+, 
then another red line will appear with the corresponding error message. By the way the concrete
syntax in~\autoref{fig:ClaimA_DSL} is for the class \inlineisar+AssertedInference+ from
the \inlineisar+ArgumentationPackage+. 

Actually the concrete syntax evaluate following the logic imposed by the ontology
defined behind the sceans. 

Unidirectional associations in class diagrams can be
semantically captured as attributes. Namely, a class diagram with two classes \inlineisar+A+ and \inlineisar+B+ with the
boolean attributes \inlineisar+attributeA+ and \inlineisar+attributeB+, and linked with an association from
\inlineisar+A+ to \inlineisar+B+ with the name \inlineisar+assoc_to_B+ is represented in \idof by:
\begin{isar}[numbers=none, backgroundcolor=\color{black!10}, frame=lines]
(*@\textcolor{Blue}{doc\_class} @*) A =           (*@ \textcolor{Blue}{doc\_class} @*) B  =
  attributeA :: bool        attributeB :: bool  
  assoc_to_B :: B
\end{isar}

In \idof we can express that a child class \inlineisar{C} inherits attributes of a class \inlineisar{A} by
\textcolor{Blue}{\inlineisar+doc_class+} \inlineisar{C = A +} \inlineisar {attributeC} \inlineisar{:: string} \dots
where the \inlineisar{+} is the inheritance arrow in class diagram. 

In our work, unidirectional associations, compositions and inheritance are the only links we need since those are the
only links used by the \sacm metamodel we capture in \idof.

of antiquotations such as the antiquotation CLAIM which is a machine verified 
hyperlink to the defined claim.... the \idof command \textcolor{Blue}{\inlineisar+text*+}. 
Recall that the latter command
represent instances of the ontology that have antiquotations providing a machine verified hyperlinks, 
machine verified references and can be updated and the updates can mechanically be traced.

In the following we encode SACM in \idof as an ontology. Our embedding implements assurance cases as meta-logical
entities in Isabelle. We are not embedding assurance arguments in the HOL logic, as this would prevent the expression of
informal reasoning and explanation. Rather, SACM is implemented as a datatype the Isabelle meta-language, meaning that
they can refer to entities like types, terms, and theorems as objects. Thus, certain claims can contain formal
expressions, but others may be unstructured natural language. Thus, we faithfully represent the inherently semi-formal
nature of assurance cases.

We focus on the \inlineisar+ArgumentationPackage+\footnote{We model all parts of argumentation, base, artifact and
  terminology packages in \idof, but omit detail of these for space reasons.} and its idea for structured arguments that
use claims, with a defined context, and supported by evidence. Claims and their relationships are modelled by the
\inlineisar+ArgumentationPackage+. Different types of evidences and context, modelled by the
\inlineisar+ArtifactPackage+, can support a claim.


Technically, the root class of the \inlineisar+ArgumentationPackage+ is \inlineisar+ArgumentAsset+, which inherits the
following base attributes from the SACM core \inlineisar+BasePackage+:
\begin{itemize}
\item \inlineisar+gid+: a unique identifier for \ac{sacm} elements.%
\item \inlineisar+isCitation+: a boolean which indicates whether an element cites another.
       \item \inlineisar+isAbstract+: a boolean which indicates whether an element is abstract or not.
\end{itemize}
The class \inlineisar+ArgumentAsset+ is represented in \idof as follows:
\begin{isar}[numbers=none, backgroundcolor=\color{black!10}, frame=lines]
(*@\textcolor{Blue}{doc\_class} @*) ArgumentAsset = ArgumentationElement +
  content_assoc:: MultiLangString 
\end{isar}
Here, \inlineisar+ArgumentationElement+ is a base class which is not discussed further. The \inlineisar+content_assoc::+
\inlineisar+MultiLangString+ is an attribute modeling an association between \inlineisar+ArgumentAsset+ and
\inlineisar+MultiLangString+ from the \inlineisar+BasePackage+. It allows classes inherited from
\inlineisar+ArgumentAsset+ to include content expressed in multiple languages, and also structured expressions, using
the \inlineisar+TerminologyPackage+. \iisar provides a similar concept in the type \inlineisar+Input.source+, which
allows us to embed a variety of informal content together with formal content utilising the Isabelle term
language. Consequently, we use \inlineisar+Input.source+ to model \inlineisar+MultiLangString+.

The class \inlineisar+ArgumentAsset+ is inherited by 3 classes: (1) \inlineisar+Assertion+, which is a unified type for
claims and their relationships; (2) \inlineisar+ArgumentReasoning+, which allows relationships between claims and their
supporting elements to explicate the argumentation strategy being employed (such as how a claim is broken down to
sub-claims); and (3) \inlineisar+ArtifactReference+, that evidences a claim with an artifact.

In \idof, \inlineisar+ArgumentAsset+ is inherited as follows:
\begin{isar}[numbers=none, backgroundcolor=\color{black!10}, frame=lines]
(*@\textcolor{Blue}{datatype}@*) assertionDeclarations_t = 
  Asserted|Axiomatic|Defeated|Assumed|NeedsSupport
(*@\textcolor{Blue}{doc\_class}@*) Assertion = ArgumentAsset +  
  assertionDeclaration::assertionDeclarations_t          
(*@\textcolor{Blue}{doc\_class}@*) ArgumentReasoning  = ArgumentAsset + 
  structure_assoc::"ArgumentPackage option"
(*@\textcolor{Blue}{doc\_class}@*) ArtifactReference = ArgumentAsset +
  referencedArtifactElement_assoc::"ArtifactElement set"
\end{isar}
Here, \inlineisar+assertionDeclarations_t+ is an \ihol enumeration type, \inlineisar+set+ is the set type, and
\inlineisar+option+ is the optional type. The attribute \inlineisar+assertionDeclaration+ is of type
\inlineisar+assertionDeclarations_t+. It allows assertions to have status \inlineisar+Asserted+, \inlineisar+Axiomatic+,
\inlineisar+Defeated+, \inlineisar+Assumed+, or \inlineisar+NeedsSupport+. The attribute \inlineisar+structure_assoc+ is
an association to the class \inlineisar+ArgumentPackage+, which is not discussed here. Finally, the attribute
\inlineisar+referencedArtifactElement_assoc+ is an association to the \inlineisar+ArtifactPackage+ allowing claims to
reference supporting artifacts.

The class \inlineisar+Claim+ is a leaf child class and inherits from the class
\inlineisar+Assertion+.  This means that an instance of \inlineisar+Claim+ has a \inlineisar+gid+, a
\inlineisar+MultiLangString+ description, and can be \inlineisar+Axiomatic+, \inlineisar+Asserted+, etc. The other child
class for \inlineisar+Assertion+ is:
\begin{isar}[numbers=none, backgroundcolor=\color{black!10}, frame=lines]
(*@\textcolor{Blue}{doc\_class}@*) AssertedRelationship = Assertion +
  isCounter::bool
  reasoning_assoc:: "ArgumentReasoning option"
\end{isar}
Here, the boolean attribute \inlineisar+isCounter+ provides a way to express if the target of the relation is a
countered or refuted by the source. The attribute \inlineisar+reasoning_assoc+ is an association to an
\inlineisar+ArgumentReasoning+, to elaborate the strategy. The class \inlineisar+AssertedRelationship+ models the
relationships between elements of type \inlineisar+ArgumentAsset+ and it is inherited by five leaf child classes:
\begin{itemize}
   \item \inlineisar+AssertedRelation+, \inlineisar+AssertedContext+: relations between 
         elements of type \inlineisar+ArgumentAsset+;
   \item \inlineisar+AssertedEvidence+: a relation that supports elements of type 
         \inlineisar+ArgumentAsset+ by artifacts+
   \item \inlineisar+AssertedArtifactSupport+, \inlineisar+AssertedArtifactContext+: are relations
         between elements of type \inlineisar+ArtifactReference+. 
\end{itemize}
In addition to the inherited attributes from parent classes,
the relationship classes have the attributes \inlineisar+source+ and \inlineisar+target+.
The source attribute carries the supporting elements and the target carries the supported elements.
Note that the concrete leaf child classes in the argumentation package are the classes: \inlineisar+Claim+,
\inlineisar+AssertedRelation+, \inlineisar+AssertedContext+, \inlineisar+AssertedEvidence+,
\inlineisar+AssertedArtifactSupport+, \inlineisar+AssertedArtifactContext+. Which is relevant
for \autoref{subsec:isacm}.

